Exploring the Origin of the Distance Bimodality of Stars in the Periphery of the Small Magellanic Cloud with APOGEE and Gaia

The Magellanic Cloud system represents a unique laboratory for study of both interacting dwarf galaxies and the ongoing process of the formation of the Milky Way and its halo. We focus on one aspect of this complex, 3 body interaction - the dynamical perturbation of the Small Magellanic Cloud (SMC) by the Large Magellanic Cloud (LMC), and specifically potential tidal effects on the SMC's eastern side. Using Gaia astrometry and the precise radial velocities and multi-element chemical abundances from APOGEE-2 DR17, we explore the well-known distance bimodality on the eastern side of the SMC. Through estimated stellar distances, proper motions, and radial velocities, we characterize the kinematics of the two populations in the bimodality and compare their properties with those of SMC populations elsewhere. Moreover, while all regions explored by APOGEE seem to show a single chemical enrichment history, the metallicity distribution function (MDF), of the "far" stars on the eastern periphery of the SMC is found to resemble that for the more metal-poor fields of the western periphery, whereas the MDF for the "near" stars on the eastern periphery resembles that for stars in the SMC center. The closer eastern periphery stars also show radial velocities (corrected for SMC rotation and bulk motion) that are, on average, approaching us relative to all other SMC populations sampled. We interpret these trends as evidence that the near stars on the eastern side of the SMC represent material pulled out of the central SMC as part of its tidal interaction with the LMC.

==> authors.tex <==
\author[0009-0000-0733-2479]{Andres Almeida}
\affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}

% \correspondingauthor{Borja Anguiano}
% \email{ba7t@virginia.edu}

% \author[0000-0001-5261-4336]{Borja Anguiano}
% \affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}


% \author[0000-0002-1793-3689]{David Nidever}
% \affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}
% \affiliation{National Optical Astronomy Observatory, 950 North Cherry Ave, Tucson, AZ 85719}

 \author{Steven R. Majewski}
 \affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}


%\correspondingauthor{Joshua T. Povick}
%\email{joshua.povick@montana.edu}

%\author{Joshua T. Povick}
%\affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}


%\author{Sten Hasselquist}
%\affiliation{Department of Physics \& Astronomy, University of Utah, Salt Lake City, UT 84112}

\author[0000-0002-1793-3689]{David L. Nidever}
\affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}

\author{Knut Olsen}

\author{Antonela Monachesi}

\author{Nitya Kallivayalil}

\author{Sten Hasselquist}



\author{Yumi Choi}

\author{Joshua Povick}

\author{John C. Wilson}
\affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}



\author{Doug Geisler}

\author{Richard R. Lane}

\author{Christian Nitschelm}

\author{Jennifer S. Sobeck}

\author{Guy S. Stringfellow}





\affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}
